Of Dice and Games: A Theory of Generalized Boosting

Cost-sensitive loss functions are crucial in many real-world prediction problems, where different types of errors are penalized differently; for example, in medical diagnosis, a false negative prediction can lead to worse consequences than a false positive prediction. However, traditional PAC learning theory has mostly focused on the symmetric 0-1 loss, leaving cost-sensitive losses largely unaddressed. In this work, we extend the celebrated theory of boosting to incorporate both cost-sensitive and multi-objective losses. Cost-sensitive losses assign costs to the entries of a confusion matrix, and are used to control the sum of prediction errors accounting for the cost of each error type. Multi-objective losses, on the other hand, simultaneously track multiple cost-sensitive losses, and are useful when the goal is to satisfy several criteria at once (e.g., minimizing false positives while keeping false negatives below a critical threshold). We develop a comprehensive theory of cost-sensitive and multi-objective boosting, providing a taxonomy of weak learning guarantees that distinguishes which guarantees are trivial (i.e., can always be achieved), which ones are boostable (i.e., imply strong learning), and which ones are intermediate, implying non-trivial yet not arbitrarily accurate learning. For binary classification, we establish a dichotomy: a weak learning guarantee is either trivial or boostable. In the multiclass setting, we describe a more intricate landscape of intermediate weak learning guarantees. Our characterization relies on a geometric interpretation of boosting, revealing a surprising equivalence between cost-sensitive and multi-objective losses.

==> 2.3-results-MO.tex <==

\subsubsection{Multiclass classification, multi-objective loss}
We now shift our focus to {\it multi-objective} losses in the multiclass setting. As seen in the binary case, a multi-objective loss function is used to control different types of errors.  Recall that the multi-objective $(\costVec, \bbz)$-learner introduced earlier in Definition \ref{def:vec_z_learner}, holds in the general multiclass setting. Then, extending the result presented in \Cref{thm:binary_MO_boost}, we now present the multiclass counterpart for boosting multi-objective learners. It is derived from both Theorems \ref{thm:main_multiclass} and \ref{prop:intro_dice_duality}, and requires a generalization of the notion of coin attainability given in \Cref{def:coin_attainability}. Thus, when there are only $2$ labels, the random guesser can be thought of as a biased coin $\bp \in \Delta_2$, whereas for general label spaces $\Y = [k]$ our random guesser corresponds to a biased dice $\bp \in \Delta_\Y$. 

\begin{definition}[{Dice attainability}]\label{def:dice_attainable}
    Let $\Y=[k]$, let $\costVec = (\cost_1,\ldots,\cost_r)$ where each $\cost_i: \Y^2 \rightarrow [0,1]$ is a cost function, let $\bz \in [0,1]^{r}$, and let $J \subseteq \Y$.
    Then $(\costVec, \bbz)$ is $J$-\emph{dice-attainable} if:
    \begin{equation}
    \label{eq:J-dice-attainable}
        \forall \bq \in \Delta_J, \ \exists \bp \in \Delta_\Y, \ \forall i = 1, \ldots, r, \qquad \cost_i(\bp,\bq) \le z_i \;.
    \end{equation}
\end{definition}
Similar to the case of coin-attainability, we again remark that the definition of dice-attainability is reminiscent of the zero-sum game given in Equation \eqref{eq:def_J_game}. A maximizing $\bq$ is chosen first, and then a minimizing  $\bp$ responds. However, here we consider a more general setting in which the payoff is vector-valued. This can be thought of as a Blackwell approachability game \citep{blackwell1956analog}, 
a  generalization of zero-sum games
 to vector payoffs.
The maximizing player here corresponds to the marginal distribution chosen by the environment over a certain subset of labels. A dice-attainable pair $(\costVec, \bbz)$ can then be guaranteed by a trivial learner which simply estimates $\bq$ from sampled data, and computes the optimal response $\bp$. Clearly, such a trivial learner exists for any class $\F$, including non-learnable classes. 




Before presenting our main result for boosting multi-objective learners, we define the following subsets of $[0,1]^r$, induced by the dice-attainability of different label subsets. Fix $\costVec = (\cost_1,\ldots,\cost_r)$ where each $\cost_i:\Y^2 \to [0,1]$ is a cost function. For every $J \subseteq \Y$ let:
\begin{equation}\label{eq:def_dice_regions_D}
    D_J(\costVec) \triangleq \left\{ \bbz  : (\costVec, \bbz) \text{ is }J\text{-dice-attainable}\right\}.
\end{equation}
First, it is easy to see that by definition we have for every $y \in \Y$ that $D_{\{y\}}(\costVec) = [0,1]^r$. Moreover, since a smaller subset $J' \subseteq J$ makes it easier for the minimizer $\bp$ to satisfy the cost-sensitive bounds in \Cref{eq:J-dice-attainable}, the following is trivially true for every $J' \subseteq J \subseteq \Y$, 
$$
 D_{J}(\costVec)  \subseteq D_{J'}(\costVec).
$$

\ym{We define only $D_J$ but use $D_i$ in the theorem. }

\begin{atheorem}[Multi-objective boosting, multiclass case]\label{thm:multiclass_MO_boost}
Let $\Y=[k]$, let $\costVec = (\cost_1,\ldots,\cost_r)$ where each $\cost_i: \Y^2 \rightarrow [0,1]$ is a cost function, and let $\bbz \in [0,1]^r$. 
Let $\threshIndex < k$ be the smallest integer for which $\bbz \notin D_{\threshIndex+1}(\costVec)$, or if none exists let $\threshIndex=k$. Then, both of the following hold. 
\begin{itemize}
    \item  {\bf\small $(\costVec, \bbz)$ is $\threshIndex$-boostable}. For every class $\F \subseteq \Y^\X$, every $(\costVec,\bbz)$-learner for $\F$ is boostable to an $\threshIndex$-List PAC learner for $\F$. 
    \item  {\bf\small $(\costVec, \bbz)$ is $\threshIndex$-dice-attainable}. As a consequence, there exists a class $\F \subseteq \Y^\X$ and a $(\costVec, \bbz)$-learner for $\F$ which cannot be boosted to an $(\threshIndex{-}1)$-List PAC learner for $\F$.
\end{itemize} 
\end{atheorem} 

 



Overall we have shown that in the multiclass cost-sensitive setting there are $k-1$ boostability thresholds $v_{{\threshIndex}}(\cost)$ which determine whether a $(\cost, z)$-learner can be boosted to a $\threshIndex$-list learner. Similarly,  there are $k-1$ boostability thresholds $v_{\overline{\threshIndex}}(\cost)$ which determine whether a $\threshIndex$-list learner can be boosted to a $(\cost, z)$-learner. 
Moreover, a similar phenomena holds in the multi-objective case, as determined by the sets $D_\threshIndex(\costVec)$, which 
 can be seen as thresholds of a higher-dimensional form, represented as a surface that separates boostable guarantees from non-boostable ones. \\
 
 


 The organization of the remainder of the paper is as follows. Section \ref{sec:binary} provides a simple boosting algorithm and analysis focused on the binary setting, proving both \Cref{thm:intro_binary_boost} and \Cref{thm:binary_MO_boost}. Section \ref{sec:duality} then provides proofs for the learner equivalence results given in \Cref{prop:intro_dice_duality} and \Cref{thm:intro_general_duality}. Then, in Section \ref{sec:multiclass} we prove all of the general results for multiclass boosting discussed above, including the main boosting results of \Cref{thm:main_multiclass} and \Cref{thm:multiclass_MO_boost}. Lastly, in Section \ref{sec:spec} we describe several natural sub-problems within the multiclass setting and provide a simplified analysis compared to the general case.

  



